Faithful and Plausible Explanations of Medical Code Predictions

Machine learning models that offer excellent predictive performance often lack the interpretability necessary to support integrated human machine decision-making. In clinical medicine and other high-risk settings, domain experts may be unwilling to trust model predictions without explanations. Work in explainable AI must balance competing objectives along two different axes: 1) Explanations must balance faithfulness to the model's decision-making with their plausibility to a domain expert. 2) Domain experts desire local explanations of individual predictions and global explanations of behavior in aggregate. We propose to train a proxy model that mimics the behavior of the trained model and provides fine-grained control over these trade-offs. We evaluate our approach on the task of assigning ICD codes to clinical notes to demonstrate that explanations from the proxy model are faithful and replicate the trained model behavior.

==> reproduceCAML.tex <==
\begin{table}[]
\begin{tabular}{lll|ll|ll}
 & \multicolumn{2}{c}{AUC} & \multicolumn{2}{c|}{F1} & \multicolumn{2}{c|}{P@n} \\ \cline{2-7} 
 & Macro & Micro & Macro & Micro & 8 & 15 \\ \hline
\multicolumn{1}{l|}{Mullenbach 2018} & 0.895 & 0.986 & 0.088 & 0.539 & 0.709 & 0.561 \\
\multicolumn{1}{l|}{Wiegreffe 2019} & 0.889 & 0.985 & 0.080 & 0.542 & 0.712 & 0.562 \\
\multicolumn{1}{l|}{Ours (using github weights)} & 0.892 & 0.978 & 0.090 & 0.298 & 0.636 & 0.471 \\
\multicolumn{1}{l|}{Ours (retraining with their code)} & 0.628 & 0.884 & 0.001 & 0.024 & 0.042 & 0.027
\end{tabular}
\end{table}
